Exploring Vision-Language Models for Open-Vocabulary Zero-Shot Action Segmentation

Temporal Action Segmentation (TAS) requires dividing videos into action segments, yet the vast space of activities and alternative breakdowns makes collecting comprehensive datasets infeasible. Existing methods remain limited to closed vocabularies and fixed label sets. In this work, we explore the largely unexplored problem of Open-Vocabulary Zero-Shot Temporal Action Segmentation (OVTAS) by leveraging the strong zero-shot capabilities of Vision-Language Models (VLMs). We introduce a training-free pipeline that follows a segmentation-by-classification design: Frame-Action Embedding Similarity (FAES) matches video frames to candidate action labels, and Similarity-Matrix Temporal Segmentation (SMTS) enforces temporal consistency. Beyond proposing OVTAS, we present a systematic study across 14 diverse VLMs, providing the first broad analysis of their suitability for open-vocabulary action segmentation. Experiments on standard benchmarks show that OVTAS achieves strong results without task-specific supervision, underscoring the potential of VLMs for structured temporal understanding.

==> sections/experiments_old.tex <==
\section{Experiments}

% \subsection{Nova: A systematic exploration of Vision Language Models for Action Segmentation}
We conduct a systematic exploration, called Nova, of the FreeSegment pipeline to investigate three key questions: 
\begin{itemize}
    \item  \textbf{VLM Exploration}: What performance do key vision–language models achieve on action segmentation tasks when integrated into the FreeSegment pipeline? 
    \item \textbf{Few Shot Exploration}: How do action segmentation performance metrics vary with the number of support videos used in FreeSegment’s few-shot stage?
    \item \textbf{Failure Mode Analysis}: What are the primary factors that constrain FreeSegment’s performance on action segmentation?
\end{itemize}

\subsection{Experimental Setup}

\textbf{Datasets.} We conduct experiments on three benchmarks widely used in action segmentation: Breakfast, GTEA, and 50Salads. For each dataset, we follow the standard splits established in prior literature. Given an evaluation split, the support videos and labels are selected from training splits.

\textbf{Evaluation Metrics.} Performance is evaluated using the following set of metrics used for reporting Action Segmentation Performance:  
\begin{itemize}
    \item F1 scores at overlap thresholds 10, 25, and 50
    \item Mean over Frames (MoF)
    \item Mean Intersection-over-Union (mIoU)
    \item Edit Distance
\end{itemize}

\textbf{Implementation.} All experiments use consistent parameter values for optimal transport as reported in \cite{xu2024temporally}. We extract features using Nvidia H200 GPU cluster using 4 GPUs. 

\subsection{VLM exploration Study}
In this study we explore 14 different VLMs from 4 family of VLMs. These 4 family of VLMs are OpenCLIP, CLIP, SigLIP and Perception Encoder. We use the VLMs as the segmentation model in SegmentFree pipeline in few shot mode, where we do not use the zero shot logits. The results are mentioned in \cref{tab:vlm_segmentation_breakfast}. These

\begin{table}[h]
\centering
\small
\caption{Exploring VLMs for SegmentFree Pipeline on Breakfast (100 frames sampled from each support video).}
\label{tab:vlm_segmentation_breakfast}
\begin{tabular}{lcccc}
\toprule
Model               & F1@10/25/50     & Edit   & Acc    & Avg   \\
\midrule
siglip-p-14-384     & 0.45 / 0.33 / 0.15 & 56.13  & 0.32   & 9.60  \\
siglip-p-16-256     & 0.47 / 0.34 / 0.16 & 57.85  & 0.33   & 9.89  \\
\addlinespace
pe-core-b16-224     & 0.46 / 0.33 / 0.15 & 56.97  & 0.32   & 9.74  \\
pe-core-l14-336     & 0.46 / 0.33 / 0.15 & 56.99  & 0.32   & 9.74  \\
\bottomrule
\end{tabular}
\end{table}


\subsection{Few Shot Exploration Study}

In the few shot exploration study we study 2 keys questions: (1.) How does performance vary with k (number of shots), and (2.) How does performance vary with number of frames sampled in each support video for the cache model. For exploring (1.) we keep the number of frames sampled at 2 values - 50. We vary k in 3 ranges - 1, 2 and 5. For exploring (2.), we keep k at the values 2 and 5, while we vary number of frames sampled as 50, 100 and 200. We select 3 best performing VLMs to report both the tables.



\begin{table}[ht]
\centering
\small
\caption{Few‐shot segmentation on Breakfast for three VLMs, stacking \(k\) values (50 frames).}
\label{tab:fewshot_k_breakfast_stack}
\begin{tabular}{l c cccc}
\toprule
Model               & $k$ & F1@10/25/50 & Edit   & Acc    \\
% \midrule
% \multirow{3}{*}{openclip-vit-l-14}
%                     & 1   & –/–/–       & –.–    & –.–    & –.–   \\
%                     & 2   & –/–/–       & –.–    & –.–    & –.–   \\
%                     & 5   & –/–/–       & –.–    & –.–    & –.–   \\
\addlinespace
\multirow{3}{*}{siglip-p-16-256}
                    & 1 & 0.43/0.30/0.13 & 53.02 & 0.32   \\
                    & 2   & 0.43/0.29/0.13   & 53.10 & 0.32    \\
                    & 5   & 0.42/0.29/0.13   & 52.22 & 0.32    \\
% \addlinespace
% \multirow{3}{*}{pe-core-g14-448}
%                     & 1   & –/–/–       & –.–    & –.–    & –.–   \\
%                     & 2   & –/–/–       & –.–    & –.–    & –.–   \\
%                     & 5   & –/–/–       & –.–    & –.–    & –.–   \\
\bottomrule
\end{tabular}
\end{table}


\subsection{Failure Mode Analysis}

To characterize where within a ground‐truth segment Vision–Language Models tend to succeed or fail, we adopt a position‐aware, chunk‐based accuracy measurement.  Formally, let
\begin{description}
  \item[\(\mathcal{G} = \{(s_g,e_g)\}_{g=1}^G\)] 
    The set of all ground‐truth segments in the test set, each spanning frames \(s_g\) to \(e_g-1\).
  \item[\(K\)] 
    Number of equal‐length chunks per segment (we use \(K=25\)).  
  \item[\(\{b_{g,k}\}_{k=0}^K\)] 
    Chunk boundaries for segment \(g\), defined by
    \[
      b_{g,k} \;=\; s_g \;+\; \Big\lfloor \tfrac{k}{K}\,(e_g - s_g)\Big\rfloor,
      \quad k = 0,\dots,K.
    \]
  \item[\(\hat y_t\)] 
    Model’s predicted action label at frame \(t\).
  \item[\(y_t\)] 
    Ground‐truth action label at frame \(t\).
  \item[\(a_{g,k}\in[0,1]\)] 
    Local chunk accuracy for segment \(g\) in chunk \(k\):
    \[
      a_{g,k}
      = 
      \frac{1}{\,|I_{g,k}|\,}
      \sum_{t\in I_{g,k}}
      \mathbf{1}\bigl[\hat y_t = y_t\bigr],
      \quad \\ 
      I_{g,k} = \{\,b_{g,k},\,b_{g,k}+1,\dots,b_{g,k+1}-1\}.
    \]
  \item[\(\bar a_k\)] 
    Mean accuracy at normalized position \(k/K\) across all segments:
    \[
      \bar a_k
      = 
      \frac{1}{G}\,
      \sum_{g=1}^G
      a_{g,k}.
    \]
  \item[\(\mathrm{AUC}_g\)] 
    Area under the chunk‐accuracy curve for segment \(g\) (normalized to \([0,1]\)):
    \[
      \mathrm{AUC}_g
      = 
      \frac{1}{K}
      \sum_{k=1}^K
      a_{g,k}.
    \]
\end{description}

\noindent
Using this setup, we compute:
\begin{itemize}
  \item The \emph{mean chunk‐accuracy curve} \(\{\bar a_k\}_{k=1}^K\), which reveals an ``$\cap$-shaped'' trend---accuracy climbs from chunk 1, peaks near the midpoint (\(\tfrac{k}{K}\approx0.4\!-\!0.5\)), then declines toward chunk \(K\).
  \item The \emph{per‐position distribution} of \(\{a_{g,k}\}\) (via boxplots), showing maximal spread (and lowest medians) at the very first (\(k=1\)) and last (\(k=K\)) chunks.
  \item The \emph{histogram of AUC values} \(\{\mathrm{AUC}_g\}\), revealing a strongly bimodal distribution with one cluster of segments yielding near-zero AUC (i.e., nearly complete failure) and another cluster near AUC~\(\approx 1\) (i.e., near-perfect recognition), with few segments in the middle.

\end{itemize}

\noindent
These metrics collectively demonstrate that VLM‐based predictions are most reliable in the \emph{interior} of action segments but suffer systematic delays at onsets and premature terminations at offsets, pinpointing the boundaries as the primary failure modes.  




\subsection{Analysis of VLM Exploration Study}

Based on the results in Table~\ref{tab:vlm_segmentation_breakfast}, we draw the following data‐driven observations:

\begin{enumerate}
  \item \textbf{Marginal Model Differences.} The four VLMs—two SigLIP variants and two PE‐Core variants—achieve nearly identical Avg scores (9.60–9.89). This suggests that the choice of underlying model has only a minor effect on segmentation quality in the few‐shot, training‐free regime.
  
  % \item \textbf{Few‐Shot Logits Dominate.} Given the small gap between models, it appears that the few‐shot support logits contribute far more to performance than variations in the VLM backbone. In other words, the inclusion of support‐set information drives the majority of the segmentation gains.
  
  \item \textbf{Encouraging Yet Limited Performance.} While obtaining F1@10 in the 0.45–0.47 range without any task‐specific training is promising, the steep decline to F1@50 (0.15–0.16) highlights substantial room for improvement—particularly in precise boundary localization.
  
  \item \textbf{F1 Trend Implications.} The sharp drop in F1 as the overlap threshold tightens indicates that FreeSegment’s temporal decoding (SMTS) struggles with fine‐grained action boundaries. This trend underscores the need for enhanced temporal smoothing or lightweight boundary refinement modules in future work.
\end{enumerate}

\noindent In summary, while FreeSegment remains fully training free and leverages few‐shot support to achieve reasonable segmentation accuracy, the near‐uniform performance across diverse VLMs and the pronounced F1 score decay reveal clear avenues for boosting boundary precision and overall segmentation fidelity.



\subsection{Analysis of Few‐Shot Exploration Study}

Table~\ref{tab:fewshot_k_breakfast_stack} shows that, for \texttt{siglip-p-16-256} on Breakfast (50 frames per support video), increasing the number of shots \(k\) from 1 to 5 yields virtually no gain—and even a slight drop—in segmentation performance:

\begin{itemize}
  \item \textbf{Flat F1 Scores.} F1@10 remains at 0.43 for \(k=1\) and \(k=2\), then decreases marginally to 0.42 at \(k=5\). F1@25 and F1@50 similarly plateau around 0.30 and 0.13, respectively.
  \item \textbf{Stable Edit and Accuracy.} Edit distance oscillates minimally (53.02 → 53.10 → 52.22) and frame‐wise accuracy holds at 0.32 across all \(k\).
\end{itemize}

These results support the hypothesis that \emph{frame‐matching can be inherently noisy when different actions exhibit similar visual patterns}. As \(k\) increases, the cache model ingests more support frames—but these additional frames do not necessarily add discriminative information. Instead, they can introduce redundant or misleading examples of visually ambiguous transitions (e.g., similar hand‐object poses across adjacent actions), which throttles any potential few‐shot gains.

In other words, simply scaling support‐set size in a training‐free pipeline does not overcome the underlying noise in per‐frame similarity: once a small, representative subset of frames is provided, adding more potentially noisy frames yields diminishing—and even negative—returns. Future work should therefore focus on \emph{filtering or weighting} support frames by their discriminative power, rather than naively increasing \(k\).  





\begin{figure*}[htbp]
  \centering
  % First row of 3 figures
  \begin{subfigure}[b]{0.25\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/qual1.png}
    \caption{Example 1: Making Sandwich.}
    \label{fig:qual1}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.25\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/qual2.png}
    \caption{Example 2: Making Fried Eggs.}
    \label{fig:qual2}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.3\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/qual3.png}
    \caption{Example 3: Preparing Coffee.}
    \label{fig:qual3}
  \end{subfigure}

  \medskip

  % Second row of 3 figures
  \begin{subfigure}[b]{0.3\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/qual4.png}
    \caption{Example 4: Preparing Pancake.}
    \label{fig:qual4}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.3\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/qual5.png}
    \caption{Example 5: Preparing Milk.}
    \label{fig:qual5}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.3\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/qual6.png}
    \caption{Example 6: Preparing Tea.}
    \label{fig:qual6}
  \end{subfigure}

  \caption{Qualitative action segmentation examples. Each subfigure shows a key frame overlaid with predicted action labels (color coded) for a different activity.}
  \label{fig:qualitative_examples}
\end{figure*}







\begin{figure*}[htbp]
  \centering
  % First row of three subfigures
  \begin{subfigure}[b]{0.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/output.png}
    \caption{Local Accuracy averaged over all classes}
    \label{fig:plot1}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/output_pour_juice.png}
    \caption{Local Accuracy for ``pour juice'' action}
    \label{fig:plot2}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/output_pour_sugar.png}
    \caption{Local Accuracy for ``pour sugar'' action}
    \label{fig:plot3}
  \end{subfigure}

  \vspace{1em}

  % Second row of three subfigures
  \begin{subfigure}[b]{0.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/output_SIL.png}
    \caption{Local Accuracy for ``backgroud'' action}
    \label{fig:plot4}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/output_take_plate.png}
    \caption{Local Accuracy for ``take plate'' action}
    \label{fig:plot5}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/output_stir_tea.png}
    \caption{Local Accuracy for ``stir tea'' action}
    \label{fig:plot6}
  \end{subfigure}

  \caption{Six‐panel figure arranged as two rows of three plots each.}
  \label{fig:two_rows_three_cols}
\end{figure*}



\begin{figure}[]
  \centering
  \includegraphics[width=0.8\linewidth]{figures/output_auc.png}
  \caption{Histogram of segment‐wise AUC values \(\{\mathrm{AUC}_g\}\), revealing a strongly bimodal distribution with peaks near 0 (complete failures) and near 1 (near‐perfect recognition).}
  \label{fig:auc_hist}
\end{figure}



\subsection{Failure Modality analysis}

\paragraph{Boundary Misalignment and Class‐Level Variations} Our position‐aware evaluation uncovers a systematic “lost at the edges” phenomenon in VLM‐based action segmentation:
\begin{itemize}
  \item \textbf{Average‐case pattern:}  
    The mean chunk‐accuracy curve rises from a low value at the segment onset (0 \%) to a peak in the interior (≈ 40–50 \%), then falls off again toward the segment offset (100 \%).  This “U‐shaped” profile indicates reliable recognition in the heart of an action but consistent misclassification right before an action begins and immediately after it ends.
  \item \textbf{Class‐specific deviations:}  
    While the broad boundary failure holds for all classes, individual actions exhibit distinct timing biases:
    \begin{itemize}
      \item \emph{pour\_juice}: almost zero accuracy up to ≈ 30 \%, then a sharp rise to ≈ 65 \%, before the usual decline.
      \item \emph{take\_plate}: low interior accuracy (≈ 6–8 \%) until the final chunks, where it jumps to ≈ 18 \%.
      \item \emph{stir\_tea}: maintains a baseline ≈ 50 \% even at edges, peaks above 80 \% mid‐segment, yet still dips at boundaries.
      \item \emph{pour\_sugar} and \emph{SIL}: near‐zero accuracy across all chunks, indicating near‐complete failure.
    \end{itemize}
  \item \textbf{All-or-nothing AUC distribution:}  
    The histogram of segment‐wise AUC values (Fig.~\ref{fig:auc_hist}) exhibits a strongly bimodal shape, with one mode at AUC≈0 (segments the model completely misses) and another at AUC≈1 (segments it nearly perfectly recognizes), and very few segments in between.  This underscores that VLMs either capture an action’s interior almost flawlessly or fail entirely when their boundary alignment is off.
\end{itemize}

Taken together, these results demonstrate that VLMs struggle to localize action boundaries precisely.  Although they capture the “core” frames of an action, they exhibit systematic onset delays and premature terminations.  Future work should therefore integrate \emph{boundary‐aware} mechanisms—such as temporal regularization or explicit onset/offset detectors—to improve VLM performance in fine‐grained action segmentation.  

\paragraph{Under‐segmentation.}
A closer look at the six qualitative examples in Figure~\ref{fig:qualitative_examples} reveals a consistent under‐segmentation tendency: in cases where the ground‐truth contains many short segments (e.g., Example (a) “Making Sandwich” with five distinct actions), the model predicts far fewer segments, effectively merging adjacent actions into a single label interval.  

% Quantitatively, we compute for each video
% \[
% \Delta_s = \bigl|\mathcal{S}_{\text{gt}}\bigr| - \bigl|\mathcal{S}_{\text{pred}}\bigr|,
% \]
% where \(\mathcal{S}_{\text{gt}}\) and \(\mathcal{S}_{\text{pred}}\) are the sets of ground‐truth and predicted segments, respectively.  Across our test set, \(\Delta_s>0\) for over 70\% of videos, confirming that the model regularly under‐segments.

We attribute this to the temporal‐consistency term in our OT‐based SMTS stage, which penalizes frequent label transitions and thus biases the solution toward fewer, longer segments.  While this smoothing improves interior accuracy, it exacerbates boundary‐smearing and leads to merged actions.  As a result, correctly capturing fine‐grained action boundaries requires more explicit boundary‐aware mechanisms—such as adaptive transition penalties or frame‐level onset/offset detectors—in future training‐free few‐shot segmentation pipelines.  


\section{Discussion}

Our Nova study highlights two core challenges for training‐free, few‐shot action segmentation with VLMs: imprecise boundary localization—evidenced by a drop from F1@10 (0.45) to F1@50 (0.15) and “U‐shaped” chunk‐accuracy profiles—and diminishing returns from larger support sets, where increasing \(k\) yields flat or even degraded performance. To overcome these limitations, we advocate three complementary refinements—introducing lightweight onset/offset detectors or adaptive transition penalties; scoring and weighting support frames by temporal distinctiveness or prototypicality; and minimal task‐specific fine‐tuning of a boundary‐refinement head atop our non‐parametric cache—to sharpen action boundaries without sacrificing the training-free ethos. In sum, FreeSegment proves that VLMs can segment “for free,” but realizing precise, real-world-grade boundaries will require these targeted, boundary-centric enhancements.


==> sections/experiments_old2.tex <==
\section{Experiments}



% Requires: \usepackage{booktabs,multirow}
% Requires: \usepackage{booktabs,multirow}
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{ll|c|c|c|c}
\toprule
\multirow{2}{*}{Category} & \multirow{2}{*}{Method} & \multicolumn{4}{c}{Metrics} \\
 &  & F1@{10,25,50} & Edit & Acc & Avg \\
\midrule
\multirow{3}{*}{Baselines} 
 & Baseline Method 1 & 5.50 / 3.13 / 1.22 & 11.43 & 5.53 & -- \\
 & Baseline Method 2 & 5.49 / 3.13 / 1.09 & 11.40 & 5.48 & -- \\
 & Random UniqueDraw & 0.00 / 0.00 / 0.00 & 0.20  & 5.46 & 1.13 \\
\midrule
\multirow{5}{*}{OpenCLIP} 
 & ViT-B/32 (Base; laion2B-s34B-b79K) & 40.75 / 30.01 / 13.16 & 77.96 & 30.66 & 38.51 \\
 & ViT-B/16 (Base; laion2B-s34B-b88K) & 41.07 / 31.05 / 13.81 & 79.18 & 31.36 & 39.29 \\
 & ViT-L/14 (Large; laion2B-s32B-b82K) & 39.22 / 29.18 / 12.40 & 76.02 & 30.37 & 37.44 \\
 & ViT-H/14 (Huge; laion2B-s32B-b79K) & 39.55 / 29.21 / 13.48 & 77.68 & 29.52 & 37.89 \\
 & ViT-g/14 (Giant; laion2B-s34B-b88K) & 39.11 / 28.75 / 12.42 & 73.73 & 30.10 & 36.82 \\
\midrule
\multirow{3}{*}{CLIP (OpenAI)}
 & ViT-B/32 (Base) & 41.84 / 31.19 / 13.84 & 88.58 & 31.30 & 41.35 \\
 & ViT-B/16 (Base) & 42.56 / 30.88 / 14.45 & 88.04 & 31.46 & 41.48 \\
 & ViT-L/14 (Large) & 41.28 / 29.97 / 13.61 & 85.45 & 30.79 & 40.22 \\
\midrule
\multirow{3}{*}{SigLIP}
 & so400m-p14-384 (Large) & 42.70 / 30.54 / 14.28 & 87.27 & 31.28 & 41.21 \\
 & so400m-p16-256-i18n (Large) & 42.59 / 31.40 / 14.06 & 88.72 & 31.49 & 41.65 \\
 & large-p16-384 (Large) & 42.37 / 31.31 / 14.24 & 87.89 & 31.38 & 41.44 \\
\midrule
\multirow{3}{*}{PE-Core}
 & B/16-224 (Base) & 39.80 / 28.38 / 13.61 & 79.07 & 30.31 & 38.24 \\
 & L/14-336 (Large) & 38.75 / 26.68 / 11.64 & 68.84 & 28.50 & 34.88 \\
 & G/14-448 (Giant) & 39.31 / 28.47 / 13.29 & 75.17 & 29.31 & 37.11 \\
\bottomrule
\end{tabular}
\caption{\textbf{50 Salads Dataset} Results of different VLMs grouped by family and model size, with baseline methods shown at the top. Baseline numbers are aggregated across all VLMs (showing average, min, and max ranges) to illustrate expected baseline variation.}
\label{tab:vlm_with_baselines}
\end{table*}




% Requires in preamble: \usepackage{booktabs,multirow}
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{ll|c|c|c|c}
\toprule
\multirow{2}{*}{Category} & \multirow{2}{*}{Method} & \multicolumn{4}{c}{Metrics} \\
 &  & F1@{10,25,50} & Edit & Acc & Avg \\
\midrule
\multirow{3}{*}{Baselines (agg.)}
 & Baseline Method 1 & 5.27 / 3.08 / 1.08 & 11.87 & 5.37 & -- \\
 & Baseline Method 2 & 5.89 / 3.36 / 1.35 & 13.15 & 5.44 & -- \\
 & Random UniqueDraw & 0.12 / 0.01 / 0.01 & 2.06 & 5.61 & 1.56 \\
\midrule
\multirow{5}{*}{OpenCLIP}
 & ViT-B/32 (Base; laion2B-s34B-b79K) & 14.72 / 9.13 / 3.77 & 37.36 & 23.52 & 17.70 \\
 & ViT-B/16 (Base; laion2B-s34B-b88K) & 15.90 / 9.95 / 3.75 & 35.33 & 20.97 & 17.18 \\
 & ViT-L/14 (Large; laion2B-s32B-b82K) & 14.07 / 8.77 / 3.30 & 35.83 & 20.94 & 16.58 \\
 & ViT-H/14 (Huge; laion2B-s32B-b79K) & 14.67 / 9.40 / 4.39 & 36.20 & 20.94 & 17.12 \\
 & ViT-g/14 (Giant; laion2B-s34B-b88K) & 15.06 / 9.81 / 3.94 & 32.52 & 20.78 & 16.42 \\
\midrule
\multirow{3}{*}{CLIP (OpenAI)}
 & ViT-B/32 (Base) & 19.68 / 13.01 / 4.92 & 44.69 & 25.60 & 21.58 \\
 & ViT-B/16 (Base) & 18.69 / 11.97 / 4.54 & 44.46 & 25.94 & 21.12 \\
 & ViT-L/14 (Large) & 17.25 / 11.44 / 4.89 & 39.55 & 24.99 & 19.62 \\
\midrule
\multirow{3}{*}{SigLIP}
 & so400m-p14-384 (Large) & 18.97 / 11.93 / 5.09 & 44.13 & 24.15 & 20.85 \\
 & so400m-p16-256-i18n (Large) & 21.08 / 13.00 / 4.93 & 51.18 & 28.29 & 23.70 \\
 & large-p16-384 (Large) & 21.33 / 13.76 / 5.44 & 51.07 & 28.08 & 23.94 \\
\midrule
\multirow{3}{*}{PE-Core}
 & B/16-224 (Base) & 15.29 / 10.28 / 3.48 & 37.01 & 22.54 & 17.72 \\
 & L/14-336 (Large) & 16.56 / 11.22 / 4.56 & 35.24 & 18.77 & 17.27 \\
 & G/14-448 (Giant) & 19.17 / 11.99 / 4.04 & 38.86 & 18.97 & 18.61 \\
\bottomrule
\end{tabular}
\caption{\textbf{GTEA Dataset} Results on the second dataset, grouped by VLM family and model size. Baseline rows at top show aggregated performance across all VLMs (averages shown; ranges omitted for brevity).\label{tab:vlm_results_dataset2}}
\end{table*}




% Requires in preamble: \usepackage{booktabs,multirow}
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{ll|c|c|c|c}
\toprule
\multirow{2}{*}{Category} & \multirow{2}{*}{Method} & \multicolumn{4}{c}{Metrics} \\
 &  & F1@{10,25,50} & Edit & Acc & Avg \\
\midrule
\multirow{3}{*}{Baselines (agg.)}
 & Baseline Method 1 & 10.75 / 6.94 / 2.84 & 14.75 & 17.48 & -- \\
 & Baseline Method 2 & 13.88 / 8.51 / 3.55 & 21.44 & 17.45 & -- \\
 & Random UniqueDraw & 0.00 / 0.00 / 0.00 & 0.72 & 17.41 & 3.63 \\
\midrule
\multirow{5}{*}{OpenCLIP}
 & ViT-B/32 (Base; laion2B-s34B-b79K) & 53.92 / 39.29 / 15.34 & 91.53 & 30.85 & 46.19 \\
 & ViT-B/16 (Base; laion2B-s34B-b88K) & 53.45 / 38.88 / 15.42 & 91.19 & 30.73 & 45.93 \\
 & ViT-L/14 (Large; laion2B-s32B-b82K) & 53.45 / 39.09 / 14.84 & 90.39 & 30.74 & 45.70 \\
 & ViT-H/14 (Huge; laion2B-s32B-b79K) & 53.74 / 39.07 / 15.20 & 90.53 & 30.70 & 45.85 \\
 & ViT-g/14 (Giant; laion2B-s34B-b88K) & 53.42 / 38.98 / 15.20 & 89.93 & 30.89 & 45.68 \\
\midrule
\multirow{3}{*}{CLIP (OpenAI)}
 & ViT-B/32 (Base) & 54.04 / 39.50 / 15.20 & 92.61 & 30.87 & 46.44 \\
 & ViT-B/16 (Base) & 53.92 / 39.52 / 15.12 & 92.48 & 30.85 & 46.38 \\
 & ViT-L/14 (Large) & 54.03 / 39.58 / 15.29 & 92.44 & 30.86 & 46.44 \\
\midrule
\multirow{3}{*}{SigLIP}
 & so400m-p14-384 (Large) & 54.26 / 39.60 / 15.34 & 92.44 & 30.89 & 46.51 \\
 & so400m-p16-256-i18n (Large) & 53.98 / 39.51 / 15.04 & 92.70 & 30.85 & 46.41 \\
 & large-p16-384 (Large) & 54.00 / 39.46 / 15.23 & 92.67 & 30.87 & 46.45 \\
\midrule
\multirow{3}{*}{PE-Core}
 & B/16-224 (Base) & 53.91 / 39.41 / 15.37 & 91.62 & 30.73 & 46.21 \\
 & L/14-336 (Large) & 53.60 / 38.77 / 15.17 & 90.01 & 30.77 & 45.66 \\
 & G/14-448 (Giant) & 53.68 / 38.92 / 15.01 & 90.94 & 30.64 & 45.84 \\
\bottomrule
\end{tabular}
\caption{Results on the Breakfast dataset, grouped by VLM family and model size. Baseline rows show aggregated performance across all VLMs (averages shown; ranges omitted for brevity).}
\label{tab:vlm_results_dataset3}
\end{table*}


% Requires in preamble: \usepackage{booktabs}
% Requires in preamble: \usepackage{booktabs,multirow}
% \begin{table}[t]
% \centering
% \renewcommand{\arraystretch}{1.2}
% \setlength{\tabcolsep}{6pt}
% \begin{tabular}{l|l|c|c|c|c|c}
% \toprule
% Dataset & Method & Acc & F1@10 & F1@25 & F1@50 & Edit \\
% \midrule
% \multirow{3}{*}{50 Salads} 
%  & Best & 31.30 & 41.84 & 31.19 & 13.84 & 88.58 \\
%  & Ablated & 5.48 & 0.17 & 0.08 & 0.03 & 0.88 \\
% \midrule
% \multirow{3}{*}{GTEA} 
%  & Best & 28.08 & 21.33 & 13.76 & 5.44 & 51.07 \\
%  & Ablated & 5.41 & 1.18 & 0.52 & 0.16 & 3.95 \\
% \midrule
% \multirow{3}{*}{Breakfast} 
%  & Best & 30.89 & 54.26 & 39.60 & 15.34 & 92.44 \\
%  & Ablated & 17.50 & 1.16 & 0.67 & 0.27 & 8.13 \\
% \bottomrule
% \end{tabular}
% \caption{Ablation Study 1: Baseline Method 0 compared with best and worst performing full models for each dataset. Dataset 1 best = OpenAI CLIP ViT-B/32, worst = PE-Core L/14-336. Dataset 2 best = SigLIP large-p16-384. Dataset 3 best = SigLIP so400m-p14-384. Placeholders remain for missing worst results in Dataset 2 and 3.}
% \label{tab:ablation1_best_worst}
% \end{table}


% % Requires in preamble: \usepackage{booktabs,multirow}
% \begin{table}[t]
% \centering
% \renewcommand{\arraystretch}{1.2}
% \setlength{\tabcolsep}{6pt}
% \begin{tabular}{l|l|c|c|c|c|c}
% \toprule
% Dataset & Method & Acc & F1@10 & F1@25 & F1@50 & Edit \\
% \midrule
% \multirow{2}{*}{50 Salads} 
%  & Best & 31.30 & 41.84 & 31.19 & 13.84 & 88.58 \\
%  & Random-ASOT & 31.53 & 6.71 & 5.16 & 2.27 & 9.35 \\
% \midrule
% \multirow{2}{*}{GTEA} 
%  & Best & 28.08 & 21.33 & 13.76 & 5.44 & 51.07 \\
%  & Random-ASOT & 17.30 & 1.38 & 0.60 & 0.25 & 17.39 \\
% \midrule
% \multirow{2}{*}{Breakfast} 
%  & Best & 30.89 & 54.26 & 39.60 & 15.34 & 92.44 \\
%  & Random-ASOT & 28.08 & 12.58 & 8.36 & 2.85 & 18.87 \\
% \bottomrule
% \end{tabular}
% \caption{Ablation Study 2: Random-ASOT compared with best performing full models for each dataset.}
% \label{tab:ablation2_random_asot}
% \end{table}
% Requires in preamble: \usepackage{booktabs,multirow}
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{4pt} % Adjust spacing for compactness
\begin{tabular}{l|cccc|cccc|cccc}
\toprule
\multirow{2}{*}{Model} 
& \multicolumn{4}{c|}{50 Salads} 
& \multicolumn{4}{c|}{GTEA} 
& \multicolumn{4}{c}{Breakfast} \\
 & F1@{10,25,50} & Edit & Acc & Avg 
 & F1@{10,25,50} & Edit & Acc & Avg
 & F1@{10,25,50} & Edit & Acc & Avg \\
\midrule
random\_uniform 
 & 0.00 / 0.00 / 0.00 & 0.20 & 5.46 & 1.13
 & 0.12 / 0.01 / 0.01 & 2.06 & 5.61 & 1.56
 & 0.00 / 0.00 / 0.00 & 0.72 & 17.45 & 3.63 \\
ES\_mean 
 & 1.49 / 0.13 / 0.04 & 5.40 & 5.63 & 2.54
 & 7.08 / 3.99 / 1.67 & 13.00 & 5.99 & 6.35
 & 20.56 / 11.97 / 3.63 & 22.39 & 17.14 & 15.14 \\
ES\_vote 
 & 2.77 / 0.84 / 0.31 & 6.72 & 5.68 & 3.26
 & 7.32 / 4.63 / 1.87 & 12.68 & 5.96 & 6.49
 & 22.15 / 13.69 / 4.52 & 24.66 & 17.15 & 16.43 \\
ES\_nrp 
 & 6.81 / 5.90 / 2.73 & 8.00 & 7.24 & 6.14
 & 7.75 / 5.35 / 2.01 & 8.29 & 12.96 & 7.27
 & 24.38 / 19.46 / 8.73 & 36.35 & 11.83 & 20.15 \\
\midrule
SigLIP-M1 
 & 42.6 / 31.4 / 14.1 & 88.7 & 31.5 & 41.7
 & 21.1 / 13.0 / 4.9 & 51.2 & 28.3 & 23.7
 & 54.0 / 39.5 / 15.0 & 92.7 & 30.9 & 46.4 \\
SigLIP-M2 
 & 42.4 / 31.3 / 14.2 & 87.9 & 31.4 & 41.4
 & 21.3 / 13.8 / 5.4 & 51.1 & 28.1 & 23.9
 & 54.0 / 39.5 / 15.2 & 92.7 & 30.9 & 46.5 \\
OpenCLIP-M1
 & 41.1 / 31.1 / 13.8 & 79.2 & 31.4 & 39.3
 & 15.9 / 10.0 / 3.8 & 35.3 & 21.0 & 17.2
 & 53.5 / 38.9 / 15.4 & 91.2 & 30.7 & 45.9 \\
CLIP-M1
 & 41.8 / 31.2 / 13.8 & 88.6 & 31.3 & 41.4
 & 19.7 / 13.0 / 4.9 & 44.7 & 25.6 & 21.6
 & 54.0 / 39.5 / 15.2 & 92.6 & 30.9 & 46.4 \\
PECore-M1
 & 39.8 / 28.4 / 13.6 & 79.1 & 30.3 & 38.2
 & 15.3 / 10.3 / 3.5 & 37.0 & 22.5 & 17.7
 & 53.9 / 39.4 / 15.4 & 91.6 & 30.7 & 46.2 \\
\bottomrule
\end{tabular}
\caption{\textbf{Comparison of baselines and five selected VLMs across three datasets} (50 Salads, GTEA, and Breakfast). Each Avg is the mean of F1@10, F1@25, F1@50, Edit, and Accuracy. Model abbreviations: SigLIP-M1 = \texttt{so400m-p16-256-i18n (Large)}, SigLIP-M2 = \texttt{large-p16-384 (Large)}, OpenCLIP-M1 = \texttt{ViT-B/16 (Base; laion2B-s34B-b88K)}, CLIP-M1 = \texttt{ViT-B/32 (Base)}, PECore-M1 = \texttt{B/16-224 (Base)}.}
\label{tab:vlm_combined_results_with_avg}
\end{table*}



% Requires: \usepackage{booktabs,multirow}
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
 & \multicolumn{3}{c|}{50 Salads} & \multicolumn{3}{c|}{GTEA} & \multicolumn{3}{c}{Breakfast} \\
Metric & Best & SMTS ($\downarrow$) & FAES ($\downarrow$) & Best & SMTS ($\downarrow$) & FAES ($\downarrow$) & Best & SMTS ($\downarrow$) & FAES ($\downarrow$) \\
\midrule
Acc   & 31.30 & 5.48 {\scriptsize (↓25.82)} & 28.53 {\scriptsize (↓2.77)} 
      & 28.08 & 5.41 {\scriptsize (↓22.67)} & 17.30 {\scriptsize (↓10.78)} 
      & 30.89 & 17.50 {\scriptsize (↓13.39)} & 26.08 {\scriptsize (↓4.81)} \\
F1@10 & 41.84 & 0.17 {\scriptsize (↓41.67)} & 6.71  {\scriptsize (↓35.13)} 
      & 21.33 & 1.18 {\scriptsize (↓20.15)} & 1.38  {\scriptsize (↓19.95)} 
      & 54.26 & 1.16 {\scriptsize (↓53.10)} & 12.58 {\scriptsize (↓41.68)} \\
F1@25 & 31.19 & 0.08 {\scriptsize (↓31.11)} & 5.16  {\scriptsize (↓26.03)} 
      & 13.76 & 0.52 {\scriptsize (↓13.24)} & 0.60  {\scriptsize (↓13.16)} 
      & 39.60 & 0.67 {\scriptsize (↓38.93)} & 8.36  {\scriptsize (↓31.24)} \\
F1@50 & 13.84 & 0.03 {\scriptsize (↓13.81)} & 2.27  {\scriptsize (↓11.57)} 
      & 5.44  & 0.16 {\scriptsize (↓5.28)}  & 0.25  {\scriptsize (↓5.19)}  
      & 15.34 & 0.27 {\scriptsize (↓15.07)} & 2.85  {\scriptsize (↓12.49)} \\
Edit  & 88.58 & 0.88 {\scriptsize (↓87.70)} & 9.35  {\scriptsize (↓79.23)} 
      & 51.07 & 3.95 {\scriptsize (↓47.12)} & 17.39 {\scriptsize (↓33.68)} 
      & 92.44 & 8.13 {\scriptsize (↓84.31)} & 18.87 {\scriptsize (↓73.57)} \\
\midrule
Avg   & 41.81 & 3.01 {\scriptsize (↓38.80)} & 10.80 {\scriptsize (↓31.01)} 
      & 23.14 & 2.64 {\scriptsize (↓20.50)} & 7.78  {\scriptsize (↓15.36)} 
      & 46.51 & 5.95 {\scriptsize (↓40.56)} & 13.75 {\scriptsize (↓32.76)} \\
\bottomrule
\end{tabular}
\caption{Ablation studies across datasets. Each block compares the Best model with SMTS (Baseline-0) and FAES (Random-ASOT). The Average row reports mean performance across Acc, F1@10, F1@25, F1@50, and Edit, with drops from Best shown using downward arrows (↓).}
\label{tab:ablation_all_datasets}
\end{table*}









% \paragraph{Datasets} The key datasets include 50 salads, Breakfast, GTEA.

% \paragraph{Implementation Details} Details related to canonical ordering and other details.

% \paragraph{Evaluation Metrics}

% \paragraph{Baseline Models} We propose 2 baselines.\\
% Baseline 1 (Anchor Based Naive Baseline): Anchor point driven segmentation. Identify anchor points, and then select midpoint of the anchor points to identify segments.
% Baseline 2 (Anchor Based DTW baseline): Dynamic time warping based version, where the canonical ordering is extracted using the high confidence classification points.

% \subsection{Explorations of VLMs in OVTAS}
% We explore OVTAS versions across different choices of Vision Language Models. And we compare those with our 2 baseline models - Anchor based Naive Baseline, Anchor Based DTW Baseline.
% Comparing OVTAS
% \subsection{Exploration of sparse OVTAS}

% \subsection{OVTAS performance by relative position in a segment}

% \subsection{Comparing with training-dependent methods}

% \section{Discussion}



















\begin{table*}[th]
\centering
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{4pt} % Adjust spacing for compactness

\caption{\textbf{Comparison of baselines and five selected VLMs across three datasets} (50 Salads, GTEA, and Breakfast). Each Avg is the mean of F1@10, F1@25, F1@50, Edit, and Accuracy. Model abbreviations: SigLIP-M1 = \texttt{so400m-p16-256-i18n (Large)}, SigLIP-M2 = \texttt{large-p16-384 (Large)}, OpenCLIP-M1 = \texttt{ViT-B/16 (Base; laion2B-s34B-b88K)}, CLIP-M1 = \texttt{ViT-B/32 (Base)}, PECore-M1 = \texttt{B/16-224 (Base)}.}
\label{tab:vlm_combined_results_with_avg}

\begin{tabular}{l|cccc|cccc|cccc}
\toprule
\multirow{2}{*}{Method} 
& \multicolumn{4}{c|}{50 Salads} 
& \multicolumn{4}{c|}{GTEA} 
& \multicolumn{4}{c}{Breakfast} \\
 & F1@{10,25,50} & Edit & Acc & Avg 
 & F1@{10,25,50} & Edit & Acc & Avg
 & F1@{10,25,50} & Edit & Acc & Avg \\
\midrule
Random
 & 0.00 / 0.00 / 0.00 & 0.20 & 5.46 & 1.13
 & 0.12 / 0.01 / 0.01 & 2.06 & 5.61 & 1.56
 & 0.00 / 0.00 / 0.00 & 0.72 & 17.45 & 3.63 \\
ES\_mean 
 & 1.49 / 0.13 / 0.04 & 5.40 & 5.63 & 2.54
 & 7.08 / 3.99 / 1.67 & 13.00 & 5.99 & 6.35
 & 20.56 / 11.97 / 3.63 & 22.39 & 17.14 & 15.14 \\
ES\_vote 
 & 2.77 / 0.84 / 0.31 & 6.72 & 5.68 & 3.26
 & 7.32 / 4.63 / 1.87 & 12.68 & 5.96 & 6.49
 & 22.15 / 13.69 / 4.52 & 24.66 & 17.15 & 16.43 \\
ES\_nrp 
 & 6.81 / 5.90 / 2.73 & 8.00 & 7.24 & 6.14
 & 7.75 / 5.35 / 2.01 & 8.29 & 12.96 & 7.27
 & 24.38 / 19.46 / 8.73 & 36.35 & 11.83 & 20.15 \\
\midrule
Ours (SigLIP-M1) 
 & 42.6 / 31.4 / 14.1 & 88.7 & 31.5 & 41.7
 & 21.1 / 13.0 / 4.9 & 51.2 & 28.3 & 23.7
 & 54.0 / 39.5 / 15.0 & 92.7 & 30.9 & 46.4 \\
Ours (SigLIP-M2) 
 & 42.4 / 31.3 / 14.2 & 87.9 & 31.4 & 41.4
 & 21.3 / 13.8 / 5.4 & 51.1 & 28.1 & 23.9
 & 54.0 / 39.5 / 15.2 & 92.7 & 30.9 & 46.5 \\
Ours (OpenCLIP-M1)
 & 41.1 / 31.1 / 13.8 & 79.2 & 31.4 & 39.3
 & 15.9 / 10.0 / 3.8 & 35.3 & 21.0 & 17.2
 & 53.5 / 38.9 / 15.4 & 91.2 & 30.7 & 45.9 \\
Ours (CLIP-M1)
 & 41.8 / 31.2 / 13.8 & 88.6 & 31.3 & 41.4
 & 19.7 / 13.0 / 4.9 & 44.7 & 25.6 & 21.6
 & 54.0 / 39.5 / 15.2 & 92.6 & 30.9 & 46.4 \\
Ours (PECore-M1)
 & 39.8 / 28.4 / 13.6 & 79.1 & 30.3 & 38.2
 & 15.3 / 10.3 / 3.5 & 37.0 & 22.5 & 17.7
 & 53.9 / 39.4 / 15.4 & 91.6 & 30.7 & 46.2 \\
\bottomrule
\end{tabular}
\end{table*}





\begin{table*}[th]
\centering
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{4pt} % Adjust spacing for compactness

\caption{\textbf{Comparison of baselines and five selected VLMs across three datasets} (50 Salads, GTEA, and Breakfast). Each Avg is the mean of F1@10, F1@25, F1@50, Edit, and Accuracy. Model abbreviations: SigLIP-M1 = \texttt{so400m-p16-256-i18n (Large)}, SigLIP-M2 = \texttt{large-p16-384 (Large)}, OpenCLIP-M1 = \texttt{ViT-B/16 (Base; laion2B-s34B-b88K)}, CLIP-M1 = \texttt{ViT-B/32 (Base)}, PECore-M1 = \texttt{B/16-224 (Base)}.}
\label{tab:vlm_combined_results_with_avg}

\begin{tabular}{l|cccc|cccc|cccc}
\toprule
\multirow{2}{*}{Method} 
& \multicolumn{4}{c|}{50 Salads} 
& \multicolumn{4}{c|}{GTEA} 
& \multicolumn{4}{c}{Breakfast} \\
 & F1@{10,25,50} & Edit & Acc & Avg 
 & F1@{10,25,50} & Edit & Acc & Avg
 & F1@{10,25,50} & Edit & Acc & Avg \\
\midrule
Random
 & 0.00 / 0.00 / 0.00 & 0.20 & 5.46 & 1.13
 & 0.12 / 0.01 / 0.01 & 2.06 & 5.61 & 1.56
 & 0.00 / 0.00 / 0.00 & 0.72 & 17.45 & 3.63 \\
ES\_mean 
 & 1.49 / 0.13 / 0.04 & 5.40 & 5.63 & 2.54
 & 7.08 / 3.99 / 1.67 & 13.00 & 5.99 & 6.35
 & 20.56 / 11.97 / 3.63 & 22.39 & 17.14 & 15.14 \\
ES\_vote 
 & 2.77 / 0.84 / 0.31 & 6.72 & 5.68 & 3.26
 & 7.32 / 4.63 / 1.87 & 12.68 & 5.96 & 6.49
 & 22.15 / 13.69 / 4.52 & 24.66 & 17.15 & 16.43 \\
ES\_nrp 
 & 6.81 / 5.90 / 2.73 & 8.00 & 7.24 & 6.14
 & 7.75 / 5.35 / 2.01 & 8.29 & 12.96 & 7.27
 & 24.38 / 19.46 / 8.73 & 36.35 & 11.83 & 20.15 \\
\midrule
Ours (SigLIP-M1) 
 & 42.6 / 31.4 / 14.1 & 88.7 & 31.5 & 41.7
 & 21.1 / 13.0 / 4.9 & 51.2 & 28.3 & 23.7
 & 54.0 / 39.5 / 15.0 & 92.7 & 30.9 & 46.4 \\
Ours (SigLIP-M2) 
 & 42.4 / 31.3 / 14.2 & 87.9 & 31.4 & 41.4
 & 21.3 / 13.8 / 5.4 & 51.1 & 28.1 & 23.9
 & 54.0 / 39.5 / 15.2 & 92.7 & 30.9 & 46.5 \\
Ours (OpenCLIP-M1)
 & 41.1 / 31.1 / 13.8 & 79.2 & 31.4 & 39.3
 & 15.9 / 10.0 / 3.8 & 35.3 & 21.0 & 17.2
 & 53.5 / 38.9 / 15.4 & 91.2 & 30.7 & 45.9 \\
Ours (CLIP-M1)
 & 41.8 / 31.2 / 13.8 & 88.6 & 31.3 & 41.4
 & 19.7 / 13.0 / 4.9 & 44.7 & 25.6 & 21.6
 & 54.0 / 39.5 / 15.2 & 92.6 & 30.9 & 46.4 \\
Ours (PECore-M1)
 & 39.8 / 28.4 / 13.6 & 79.1 & 30.3 & 38.2
 & 15.3 / 10.3 / 3.5 & 37.0 & 22.5 & 17.7
 & 53.9 / 39.4 / 15.4 & 91.6 & 30.7 & 46.2 \\
\bottomrule
\end{tabular}
\end{table*}

==> sections/method_2.tex <==
\section{Method}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/TPGAS_pipeline.pdf}
  \caption{ Open-Vocabulary Temporal Action Segmentation (OVTAS) Pipeline. Our 2 stage pipeline adopts a "segmentation by classification" approach to tackle temporal action segmentation (TAS). The first stage, Frame-Action Embedding Similarity (FAES) generates a cost matrix by matching frames with action labels. The second stage, Similarity-Matrix driven Action Segmentation (SMTS) tackles the temporal inconsistency observed in stage 1, and generates temporally consistent action segments.  }
  \label{fig:tpgas_pipeline}
\end{figure}

\subsection{Terminology}

\noindent\textbf{Notation.} 
Bold uppercase = matrices, bold lowercase = vectors, italics = scalars. 
Let $T$ be the number of frames, $N$ the number of action labels, and $C$ the embedding dimension.

\begin{description}
  \item[A (Activity)] 
  A high-level category for an entire video (e.g., ``making tea'').

  \item[$\mathbf{X}\in\mathbb{R}^{T\times C}$ (Frame Embeddings)] 
  Row-wise $\ell_2$-normalized frame embeddings from the VLM vision encoder; 
  $\|\mathbf{x}_t\|_2=1$.

  \item[$\mathbf{A}\in\mathbb{R}^{N\times C}$ (Action Embeddings)] 
  Row-wise $\ell_2$-normalized text embeddings for the $N$ action labels from the VLM text encoder; 
  $\|\mathbf{a}_n\|_2=1$.

  \item[$\mathbf{S}\in\mathbb{R}^{T\times N}$ (Similarity / Logit Matrix)] 
  Cosine similarity (dot product) between frame and action embeddings:
  \[
    \mathbf{S} = \mathbf{X}\,\mathbf{A}^\top, 
    \quad \ell_t = \mathbf{x}_t\,\mathbf{A}^\top \in \mathbb{R}^{1\times N}.
  \]

  \item[$\mathbf{P}\in\mathbb{R}^{T\times N}$ (Frame Classification Probabilities)] 
  Row-wise softmax over actions:
  \[
    \mathbf{P} = \mathrm{softmax}_N(\mathbf{S}), 
    \quad \mathbf{p}_t = \mathrm{softmax}(\ell_t).
  \]
\end{description}

\subsection{Preliminaries}

\paragraph{(Entropic / Unbalanced) Optimal Transport.}
Given similarity $\mathbf{S}\in\mathbb{R}^{T\times N}$, define the cost $\mathbf{C} = \mathbf{1}-\mathbf{S}$. 
Let
\[
\mathbf{u} = \tfrac{1}{T}\mathbf{1}_T,
\quad 
\mathbf{v} = \tfrac{1}{N}\mathbf{1}_N.
\]

The balanced, entropic OT problem is
\begin{multline}
\Pi^* = \arg\min_{\Pi\in U(\mathbf{u},\mathbf{v})}
   \;\langle \Pi,\mathbf{C}\rangle \\
   - \;\varepsilon H(\Pi),
\end{multline}
where 
\(
U(\mathbf{u},\mathbf{v})=\{\Pi\!\ge\!0:\Pi\mathbf{1}=\mathbf{u},\;\Pi^\top\mathbf{1}=\mathbf{v}\}.
\)

% The unbalanced variant relaxes marginals with KL penalties:
% \begin{multline}
% \Pi^* = \arg\min_{\Pi\ge 0}\;
%    \langle \Pi,\mathbf{C}\rangle - \varepsilon H(\Pi) \\
%    + \lambda_r\,\mathrm{KL}(\Pi\mathbf{1}\,\|\,\mathbf{u})
%    + \lambda_c\,\mathrm{KL}(\Pi^\top\mathbf{1}\,\|\,\mathbf{v}).
% \end{multline}

We denote this operator abstractly as $\Pi^*=\mathcal{G}(\mathbf{S})$.

\subsection{Stage 1: Frame–Action Embedding Similarity (FAES)}

FAES computes raw similarity scores between frame and action embeddings:
\begin{enumerate}
  \item \textbf{Embed frames and actions.} 
  Obtain $\mathbf{X}\in\mathbb{R}^{T\times C}$ and $\mathbf{A}\in\mathbb{R}^{N\times C}$; 
  apply row-wise $\ell_2$-normalization.

  \item \textbf{Compute similarities (logits).} 
  \[
    \mathbf{S} = \mathbf{X}\,\mathbf{A}^\top \in \mathbb{R}^{T\times N}, 
    \quad \ell_t=\mathbf{x}_t\mathbf{A}^\top.
  \]

\subsection{Stage 2: Similarity Matrix–driven Temporal Segmentation (SMTS)}

SMTS consumes the similarity matrix $\mathbf{S}$ and produces temporally consistent segments:
\begin{enumerate}
  \item \textbf{Temporal Prior Construction.} 
  Build a diagonal-banded prior:
  \[
    R_{ij} = \Bigl\lvert \tfrac{i}{T} - \tfrac{j}{N}\Bigr\rvert,
  \]
  encouraging alignment between early frames and early actions.

  \item \textbf{OT Alignment.} 
  With $\mathbf{S}\in\mathbb{R}^{T\times N}$ and cost 
  \[
    \mathbf{C} = \mathbf{1} - \mathbf{S},
  \]
  solve
  \begin{multline}
    \Pi^* = \arg\min_{\Pi\in U(\mathbf{u},\mathbf{v})}
       \;\langle \Pi,\,\mathbf{C}+\rho R\rangle \\
       - \;\varepsilon \sum_{i,j}\Pi_{ij}\log\Pi_{ij},
  \end{multline}
  where $\mathbf{u}=\tfrac{1}{T}\mathbf{1}_T$, $\mathbf{v}=\tfrac{1}{N}\mathbf{1}_N$.

 $\rho>0$ is a scalar that weights the temporal prior $R$ in the OT objective. $\rho=0$ removes the prior from the optimization objective.

  \item \textbf{Action Segmentation.} 
  Assign each frame $t$ the action with maximum OT mass:
  \[
    \hat y_t = \arg\max_{j}\,\Pi^*_{t,j}.
  \]
\end{enumerate}
\end{enumerate}

